SAT-based Analysis of Large Real-world Feature Models is Easy

Modern conflict-driven clause-learning (CDCL) Boolean SAT solvers provide efficient automatic analysis of real-world feature models (FM) of systems ranging from cars to operating systems. It is well-known that solver-based analysis of real-world FMs scale very well even though SAT instances obtained from such FMs are large, and the corresponding analysis problems are known to be NP-complete. To better understand why SAT solvers are so effective, we systematically studied many syntactic and semantic characteristics of a representative set of large real-world FMs. We discovered that a key reason why large real-world FMs are easy-to-analyze is that the vast majority of the variables in these models are unrestricted, i.e., the models are satisfiable for both true and false assignments to such variables under the current partial assignment. Given this discovery and our understanding of CDCL SAT solvers, we show that solvers can easily find satisfying assignments for such models without too many backtracks relative to the model size, explaining why solvers scale so well. Further analysis showed that the presence of unrestricted variables in these real-world models can be attributed to their high-degree of variability. Additionally, we experimented with a series of well-known non-backtracking simplifications that are particularly effective in solving FMs. The remaining variables/clauses after simplifications, called the core, are so few that they are easily solved even with backtracking, further strengthening our conclusions.

==> acknowledgement.tex <==
\section{Acknowledgement}

We thank Saket Saurabh for pointing out the connection to the dual
of strong backdoors in Theorem~\ref{backdoorconn}.

==> theory.tex <==
\section{Finding restricted variables and connections to backdoors}
As defined in the introduction, we call a variable $v$ of a satisfiable CNF formula $\phi$ {\it unrestricted} with respect to a partial assignment $S$, if $S$ can be completed to a satisfying assignment to $\phi$ with $v=0$ and a satisfying assignment with $v=1$. We call a variable {\it unrestricted} (without reference to any partial assignment) if there exists a partial assignment $S$ for which the variable is unrestricted and we call it {\it restricted} otherwise.

Note that if a CDCL algorithm picks the partial assignment $S$ correctly, then it will not backtrack on an unrestricted variable, and we believe that this is what is happening in the solvers when solving feature models, as there are overwhelmingly many unrestricted variables.
%It is easy to justify theoretically that if there are very few restricted variables in $\phi$, then one can find a satisfying assignment fast, as the following theorem shows. The proofs will be available in the tech report.
%\begin{theorem} 
%\label{complexity}
%If a Boolean CNF formula $F$ on $n$ variables and $m$ clauses, has at most $k$ restricted variables, then its satisfiability can be tested in $O(2^k f(n,m))$ time where $f$ is a polynomial function.
%\end{theorem}
%\begin{proof}
%A Davis-Putnam algorithm that branches on each variable will not backtrack on the unrestricted variables, as they can be `completed' to a satisfying assignment. Hence such an algorithm will only make $O(2^k)$ steps each taking a polynomial time (to instantiate and simplify the formula).
%\end{proof}
%
%Unlike the backdoor based approach to satisfiability~\cite{BackdoorsInLearning,WilliamsBackdoors,szeider2005backdoor,misra2013upper} which involves finding a small set of backdoor variables, and then trying various assignments for the backdoor variables to test satisfiability, we observe that a large set of unrestricted variables can explain the (fast) satisfiability method for a class of formulas, where we {\it do not need} to find them. I.e., just the mere existence of a large set of unrestricted variables in a formula implies that the satisfiability can be tested fast. We believe that this can give a possible explanation for fast testability of satisfiability of a large class of CNF formulas.

Here we find interesting connections between this parameter (of the number of restricted variables) and the well studied parameter of the number of backdoor variables. Let $\mathcal(C)$ be a class of CNF formulas. Recall~\cite{WilliamsBackdoors,gaspers2012backdoors} that a {\it strong $\mathcal(C)$ backdoor} of a Boolean formula $F$ is a set $B$ of variables such that every assignment to the set $B$ of variables (and simplification of $F$ with the assignment) results in a formula in $\mathcal(C)$. A {\it weak $\mathcal(C)$ backdoor} of $F$ is a set $B$ of variables such that there exists an assignment to the variables of $B$ such that the resulting simplified formula is satisfiable and is in $\mathcal(C)$. We observe the following interesting connections for the set of unrestricted variables with backdoors.

Let $E$ be the empty formula which is trivially satisfiable. Let $S$ be the class of all satisfiable CNF formulas. Then we show the following.
\begin{theorem}
\label{backdoorconn}
A CNF formula $F$ with $n$ variables has at most $k$ restricted variables if and only if
it has a weak $E$ backdoor of size at most $k$ and if and only if
it has a strong $S$ backdoor of size at least $n-k$.
\end{theorem}
%\begin{proof}
%Let $F$ have a set $B$ of at most $k$ restricted variables. Consider the assignment for the $k$ variables of $B$ that makes $F$ satisfiable.
%Now we claim that once we simplify the formula with the assignment, the resulting formula $F'$ must be empty (i.e. $F'=E$). Suppose on the contrary $F'$, has a non-empty clause with variables $v_1, v_2, \ldots v_l$ ($l$ could be $1$). As all the variables $v_1$ to $v_l$ are unrestricted, there is a satisfying assignment that sets all the variables to $0$. But setting all of them $0$ does not satisfy the resulting formula $F'$, a contradiction. Thus $B$ is a weak $E$ backdoor set of size at most $k$. Conversely if $B$ is a weak $E$ backdoor, then there is an assignment to the variables of $B$ that results in an empty clause, and hence the remaining at least $n-k$ variables can be set in any way and hence unrestricted. Thus $F$ has at most $k$ restricted variables.
%
%To show connections to strong $S$ backdoor, consider the unrestricted variables $U$ of $F$. By definition, every assignment to the variables of $U$ results in a satisfiable formula on the at most $k$ variables (or some subset) of $B$, and hence they form a strong $S$ backdoor set.
%Conversely if $B$ is a strong $S$ backdoor set, as every assignment to the variables of $B$ results in a satisfying formula, $B$ is an unrestricted set of variables.
%\end{proof}

By a reduction from the Hitting Set problem, it can be shown that finding weak $E$ backdoor of size at most $k$ is not only $NP$-complete, but complete for the parameterized complexity class $W[2]$ for general CNF formulas. However it is fixed-parameter tractable (but still $NP$-complete) for $d$-CNF formulas where each clause length is bounded by a fixed constant $d$.  As we could not find a theorem for this 
in the backdoor literature~\cite{gaspers2012backdoors,misra2013upper,szeider2005backdoor} we give a theorem for completeness.
\begin{theorem}
Determining if a given formula on $n$ variables has a weak $E$ backdoor of size at most $k$ is $W[2]$-complete for general formulas, and 
is fixed-parameter tractable with an $O^*(d^k)$ algorithm for $d$-CNF formulas~\footnote{The $O^*()$ notation ignores polynomial factors, i.e., by $O^*(d^k)$ we mean $O(d^k n^c)$ for some constant c. This is standard in parametrized complexity.}.
\end{theorem}
%\begin{proof}
%Recall that in the hitting set problem, we are given a universe set $A$ of size $n$, a family $\mathcal{F}$ of subsets of $A$, and the goal is to find a subset $B$ of $A$ of size at most $k$ such that $B \cap F \neq \empty$ for every $F \in \mathcal{F}$. This problem is known to be $NP$-complete even if every set in $\mathcal{F}$ is of size $2$ (as it is the same as the famous {\sc vertex cover} problem).
%
%To reduce this problem to the problem of finding a weak $E$ backdoor set of a formula, do the natural transformation of creating a literal for every element of $A$, and making every set of $F$ a disjunction of the (pure) variables corresponding to the elements of the set. The formula $F'$ is a conjunction of all the disjunctions corresponding to the sets of $\mathcal{F}$. Now if $\mathcal{F}$ has a hitting set of size at most $k$, then if we set the corresponding variables $1$ and simplify the formula, then what results is an empty formula, and hence those set of $k$ variables form a weak $E$ backdoor set of size at most $k$. Conversely, if the formula $F'$ has a weak $E$ backdoor set of size at most $k$, then as there is a setting for these variables that results in an empty formula, these $k$ variables must have a non-empty intersection with every clause, and hence with every set of $\mathcal{F}$.
%
%To show fixed-parameter tractability for a $d$-CNF formula $F$, consider a clause of $F$ with $d$ variables. At least one of the variables of the clause must be in a weak $E$ backdoor set (as otherwise, this clause will remain after setting the weak backdoor variables and simplifying).
%Thus we can design a `branching' algorithm which branches by picking one of the variables in each branch as a weak backdoor variable and recursively testing whether the resulting formula has a weak backdoor $E$ set of size at most $k-1$. This results in a $d$-way branch with $O(d^k)$ 
%branching tree. In the leaves, we are interested in testing whether there is a weak backdoor $E$ set of size $0$. This is the same as testing whether the resulting formula is empty which can be tested in polynomial time.
%\end{proof}
By Theorem~\ref{backdoorconn}, it follows that
\begin{corollary}
Determining if a given formula on $n$ variables, has at most $k$ restricted variables or at least $n-k$ strong $S$ backdoor set is $W[2]$-complete for general formulas, and is fixed-parameter tractable with an $O^*(d^k)$ algorithm for $d$-CNF formulas.
\end{corollary}

The proofs are omitted due to lack of space, and are available in the tech report: http://arxiv.org/abs/1506.05198.
%As noted earlier, Theorem~\ref{complexity} did not require that the set of restricted variables be found efficiently, so the complexify of finding the set of restricted variables has no effect on the complexity of satisfiability (unlike the case of backdoor variables) of the formulas having a small set of restricted variables. Due to Theorem~\ref{backdoorconn}, this observation (that we don't need to find them to test satisfiability) is true when there is a small set of weak $E$ backdoor variables as well as when there are a large number of strong $S$ backdoor 
%sets. While there has been a lot of literature on backdoor sets, we do not know whether these interesting observations have been made before.

